Cross-Matched Interval Prevalence of High Dimensional Point Clouds

Topological Data Analysis (TDA) has been applied with success to solve problems across many scientific disciplines. However, in the setting of a point cloud $X$ sampled from a shape $\mathcal{S}$ of low intrinsic dimension embedded within high ambient dimension $\mathbb{R}^D$, persistent homology, a key element to many TDA pipelines, suffers from two problems. First, when relatively small amounts of noise are introduced to the point cloud, persistent homology is unable to recover the true shape of $\mathcal{S}$. Secondly, the computational complexity of persistent homology scales poorly with the size of a point cloud. Although there is recent work that addresses the first issue via topological bootstrapping methods and topological prevalence, these new techniques still fall victim to the second issue. Here we introduce the cross-matched prevalence image (CMPI), an image which approximates the topological prevalent information of said point cloud, requiring only computations of persistent homology on the scale of samples of the point cloud and not the entire point cloud itself. We compute the CMPI for high dimensional synthetic data, demonstrating that it performs similarly in noise robustness experiments and accurately captures prevalent topological features as compared to previous topological bootstrapping methods.

==> sec/8_bib.tex <==
\begin{thebibliography}{}
\setlength{\itemindent}{-\leftmargin}
\makeatletter\renewcommand{\@biblabel}[1]{}\makeatother

\bibitem{Adams} Adams, H., T.~Emerson, M.~Kirby, R.~Neville, C.~Peterson, P.~Shipman, S.~Chepushtanova, E.~Hanson, F.~Motta, L.~Ziegelmeier (2017).
	\newblock Persistence Images: A Stable Vector Representation of Persistent Homology
	\newblock Journal of Machine Learning Research 18 1-35.
	
\bibitem{Ahmed} Ahmed, M., B.~Fasy, and C.~Wenk (2014). 
	\newblock Local persistent homology based distance between maps. 
	\newblock In SIGSPATIAL. ACM, Nov. 2014

\bibitem{PersLay} Carriere, M., F.~Chazal, Y.~Ike, T.~Lacombe, M.~Royer, Y.~Umeda (2020).
	\newblock PersLay: A Neural Network Layer for Persistence Diagrams and New Graph Topological Signatures.  					\newblock Proceedings of the Twenty Third International Conference on Artificial Intelligence and Statistics, PMLR 108:2786-2796.
	
\bibitem{Deq} Dequ´eant, M., S.~Ahnert, H.~Edelsbrunner, T.~Fink, E.~Glynn, G.~Hattem,
A.~Kudlicki, Y.~Mileyko, J.~Morton, A.~Mushegian, L.~Pachter, M.~Rowicka, A.~Shiu,
B.~Sturmfels, and O.~Pourqui´e (2008)
	\newblock Comparison of pattern detection methods in microarray time series of the segmentation clock. 
	\newblock PLoS ONE, 3(8):e2856.

\bibitem{Easley} Easley, T., K.~Freese, E.~Munch, J.~Bijsterbosch (2023).
	\newblock Comparing representations of high-dimensional data with persistent homology: a case study in neuroimaging.
	\newblock arXiv 2306.13802.
	


\bibitem{ELZ} Edelsbrunner, H., D.~Letscher, and A.~Zomorodian (2000).
	\newblock Topological persistence and simplification.
	\newblock In Foundations of Computer Science. Proceedings. 41st Annual Symposium on, pages 454-463.

\bibitem{GR} Garcia-Redondo, I., A.~Monod, and A.~Song (2024).
    \newblock Fast Topological Signal Identification and Persistent Cohomological Cycle Matching.
    \newblock Journal of Applied and Computational Topology 8, 695-726.
    
\bibitem{Headd} Headd, J., Y.E.~Ban, P.~Brown, H.~Edelsbrunner, M.~Vaidya, J.~Rudolph (2007).
	\newblock Protein-protein interfaces: properties, preferences, and projections.
	\newblock Journal of Proteome Research, 6(7): 2576-2586.
	\newblock PMID: 1754262
	
\bibitem{Hensel} Hensel, F., M.~Moor, B.~Rieck (2021).
	\newblock A Survey of Topological Machine Learning Methods
	\newblock Frontiers in Artificial Intelligence vol 4.

\bibitem{Hu} Hu, X., F.~Li, D.~Samaras, and C.~Chen (2019).  
	\newblock Topology-preserving deep image segmentation.
	\newblock In Advances in Neural Information Processing Systems, 5658–5669.

\bibitem{ellipse} Jin, Y. (2022).
	\newblock ellipse (version 0.6.0)
	\newblock https://pypi.org/project/ellipse/

\bibitem{Li} Li, C., M.~Ovsjanikov, and F.~Chazal (2014). 
	\newblock Persistence-based structural recognition. 
	\newblock In Computer Vision and Pattern Recognition (CVPR), 2014 IEEE Conference on, pages 2003–2010, June 2014.
	
\bibitem{Otter} Otter, N., M.A.~Porter, U.~Tillmann et al.(2017)
	\newblock A roadmap for the computation of persistent homology.
	\newblock EPJ Data Sci. 6, 17
	
\bibitem{Reani} Reani, Y., O.~Bobrowski (2023).
    \newblock Cycle Registration in Persistent Homology with Applications in Topological Bootstrap.
    \newblock IEEE Transactions on Pattern Analysis and Machine Intelligence, vol. 45, no. 5, pp. 5579-5593, 1 May 2023.
	
\bibitem{Verri} Verri, A., C.~Uras, P.~Frosini, M.~Ferri (1993).
	\newblock On the use of size functions for shape analysis.
	\newblock Biological Cybernetics, 70, 99-107.
\end{thebibliography}
